Multi-Agent VQA: Exploring Multi-Agent Foundation Models in Zero-Shot Visual Question Answering

This work explores the zero-shot capabilities of foundation models in Visual Question Answering (VQA) tasks. We propose an adaptive multi-agent system, named Multi-Agent VQA, to overcome the limitations of foundation models in object detection and counting by using specialized agents as tools. Unlike existing approaches, our study focuses on the system's performance without fine-tuning it on specific VQA datasets, making it more practical and robust in the open world. We present preliminary experimental results under zero-shot scenarios and highlight some failure cases, offering new directions for future research.

==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related}

% \begin{figure*}[t]
%   \centering
%     \includegraphics[width=1\linewidth]{figs/pipeline.png}
%     \caption{Overview of the Adaptive Multi-Agent VQA System. The process begins with an LVLM attempting to answer a visual question directly. Upon encountering object detection challenges, an LLM agent identifies necessary objects, which are then processed by a specialized object-detection agent. A similar approach is applied for counting tasks. Subsequently, the LVLM reattempts the question, with the response assessed by LLM-based graders.} \vspace{-5mm}
%     \label{fig:pipeline}
% \end{figure*}

% \paragraph{Foundation models, multi-agents, and using tools}


% \paragraph{Visual question answering}
